Accelerating Cosmic Microwave Background map-making procedure through preconditioning

Estimation of the sky signal from sequences of time ordered data is one of the key steps in Cosmic Microwave Background (CMB) data analysis, commonly referred to as the map-making problem. Some of the most popular and general methods proposed for this problem involve solving generalised least squares (GLS) equations with non-diagonal noise weights given by a block-diagonal matrix with Toeplitz blocks. In this work we study new map-making solvers potentially suitable for applications to the largest anticipated data sets. They are based on iterative conjugate gradient (CG) approaches enhanced with novel, parallel, two-level preconditioners. We apply the proposed solvers to examples of simulated non-polarised and polarised CMB observations, and a set of idealised scanning strategies with sky coverage ranging from nearly a full sky down to small sky patches. We discuss in detail their implementation for massively parallel computational platforms and their performance for a broad range of parameters characterising the simulated data sets. We find that our best new solver can outperform carefully-optimised standard solvers used today by a factor of as much as 5 in terms of the convergence rate and a factor of up to $4$ in terms of the time to solution, and to do so without significantly increasing the memory consumption and the volume of inter-processor communication. The performance of the new algorithms is also found to be more stable and robust, and less dependent on specific characteristics of the analysed data set. We therefore conclude that the proposed approaches are well suited to address successfully challenges posed by new and forthcoming CMB data sets.

==> sections_post_sub/app_coarse_space_alt.tex <==
%!TEX root = ../midas_preconditioner_post_sub.tex 

\section{Krylov Methods}\label{sec:krylov_methods} % (fold)

Since there is no universally agreed upon definition, we define here that a \emph{Krylov method} solves $\mathbf{A} \vec{x} = \vec{b}$ by repeatedly performing matrix-vector multiplications involving $\mathbf{A}$. Starting with initial guess $\vec{x}_{0}$, a Krylov method bootstrap its way up to more accurate approximation $\vec{x}_{m}$ to a desired solution. In iteration $m$ a Krylov method produces an approximate solution $\vec{x}_{m}$ from a \emph{Krylov space} generated by a vector $\vec{c}$,
\begin{eqnarray}\label{eq:krylov_space}
        \mathcal{K}_{m}( \mathbf{A} , \vec{c}) = \text{SPAN}\left\{ \vec{c},\mathbf{A}\vec{c},\ldots,\mathbf{A}^{m-1}\vec{c}\right\}.
\end{eqnarray}

A popular choice is $\vec{c}= \vec{b} - \mathbf{A}\vec{x}_{0}=\vec{r}_{0}$. That is why we restrict ourselves to Krylov spaces $\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$ that are generated by the residual $\vec{r}_{0}$ of a linear system $\mathbf{A} \vec{x}_{0} = \vec{b}$.

\subsection*{GMRES - An Example of a Krylov Method}\label{sub:gmres_an_example_of_a_krylov_method} % (fold)

In iteration $m>0$, the generalized minimal residual method (GMRES)~\citep{gmres86}   picks the 'best' solution $\vec{x}_m$ from the Krylov space $\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$. 'Best' means here, that $\vec{x}_{m} = \vec{x}_{0} + \vec{z}_{m}$ with $\vec{z}_{m}\in\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$ solves the least squares problem
\begin{equation}\label{eq:lq_gmres}
	\vec{z}_{m} = \min_{z\in\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})} \|\vec{b} -\mathbf{A}(\vec{x}_{0} + \vec{z})\|
\end{equation}
in the Euclidian norm $\|\cdot\|$. GMRES solves this least squares problem by constructing an orthogonal basis $\{ \vec{w}_{1}, \vec{w}_{2}, \ldots, \vec{w}_{m}\}$ for $\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$ using \emph{Arnoldi's method} (see algorithm~\ref{algo:arnoldi}), which is a version of the Gram-Schmidt procedure tailored to Krylov spaces. Starting with the normalized initial residual $\vec{w}_{1} = \vec{r}_{0}/\|\vec{r}_{0}\|$ as a basis for $\mathcal{K}_{1}(\mathbf{A},\vec{r}_{0})$, Arnoldi's method recursively builds an orthonormal basis for $\mathcal{K}_{m+1}(\mathbf{A},\vec{r}_{0})$ from $\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$ by orthogonalizing the vector $\mathbf{A}\vec{w}_{m}$ from $\mathcal{K}_{m+1}(\mathbf{A},\vec{r}_{0})$ against the previous space $\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$.That is, 
\begin{equation}
	\hat{\vec{w}}_{m+1} = \mathbf{A}\vec{w}_{m} - (h_{1m}\vec{w}_{1}+\ldots+h_{mm}\vec{w}_{m}),
\end{equation}
where $h_{mm} = (\mathbf{A}\vec{w}_{m},\vec{w}_{m}) = \vec{w}^{\dagger}_{m}\mathbf{A}\vec{w}_{m}$ and $\dagger$ denotes the conjugate transpose. The new basis vector is
\begin{equation}
	\vec{w}_{m+1} = \hat{\vec{w}}_{m+1}/\|\hat{\vec{w}}_{m+1}\|.
\end{equation}
If we collect the orthonormal basis vectors for $\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$ in a matrix, $\mathbf{W}_{m} = (\vec{w}_{1}\ldots\vec{w}_{m})$, we get the decomposition associated with Arnoldi's method:
\begin{equation}\label{eq:arnoldi_fundamental}
	\mathbf{A}\mathbf{W}_{m} = \mathbf{W}_{m+1}\bar{\mathbf{H}}_{m},
\end{equation}
where $\bar{\mathbf{H}}_{m}$ is an upper Hessenberg matrix of a size $(m+1)\times m$ (an upper triangular matrix with an additional off-diagonal below the diagonal).

\begin{algorithm}
\caption{Basic Arnoldi Algorithm
}
\begin{algorithmic}[1]
\REQUIRE $\mathbf{A},\,\vec{r}_{0}$,\,$\vec{w}_{1} = {\vec{r}_{0}}/{||\vec{r}_{0}||}$
\FOR{$j = 1 \to m$}
	\FOR{$i = 1 \to j$}
		\STATE $h_{i,j} = (\mathbf{A}\vec{w}_{j},\vec{w}_{i})$
	\ENDFOR  
	\STATE $\vec{v}_{j} = \mathbf{A}\vec{w}_{j} - \sum\limits_{i = 1}^{j}h_{i,j}\vec{w}_i$
	\STATE $h_{j+1,j} = || \vec{v}_{j} ||$ 
	\STATE $\vec{w}_{j+1} = \vec{v}_{j} / h_{j+1,j}$
\ENDFOR
\end{algorithmic}
\label{algo:arnoldi}
\end{algorithm}

In the context of the least squares problem~\eqref{eq:lq_gmres} this means: If $\vec{z}\in\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$, then $\vec{z} = \mathbf{W}_{m}\vec{y}$ for some $\vec{y}$, so
\begin{equation}
	\mathbf{A}\vec{z}=\mathbf{A}\mathbf{W}_{m}\vec{y}=\mathbf{W}_{m+1}\bar{\mathbf{H}}_{m}\vec{y}\;\text{and}\;\vec{r}_{0}=\beta\vec{w}_{1} = \beta\mathbf{W}_{m+1}\vec{e}_{1},
\end{equation}
where $\beta=\|\vec{r}_{0}\|$ and $\vec{e}_{1}$ is the first column of the identity matrix. The least square problem in iteration $m$ of $GMRES$ reduces to much smaller minimization problem
\begin{equation}
	\min_{z\in\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})} \|\vec{b} -\mathbf{A}(\vec{x}_{0} + \vec{z})\| = \min_{y} \| \beta \vec{e}_{1} - \bar{\mathbf{H}}_{m}\vec{y}\|.
\end{equation}
Future more, the approximate solution at the \emph{m}-th iteration, denoted by $\vec{x}_{m}$, is then contained in the affine subspace $\vec{x}_{0}+\mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})$, i.e., 
\begin{equation}
	\vec{x}_{m} \in \vec{x}_{0} + \mathcal{K}_{m}(\mathbf{A},\vec{r}_{0})
\end{equation} 
Finally, in Algorithm~\ref{algorithm:gmres} you will find complete GMRES proceedure.
\begin{algorithm}
\caption{Basic GMRES Algorithm}
\begin{algorithmic}[1]\label{algorithm:gmres}
\REQUIRE $\vec{r}_{0}=b-\mathbf{A}\vec{x}_{0},\,\beta=\|\vec{r}_{0}\|,\,\vec{w}_{1} = {\vec{r}_{0}}/{\beta}$
\FOR{$j = 1 \to m$}
	\STATE $\vec{v}_{j} = \mathbf{A}\vec{w}_{j}$
	\FOR{$i = 1 \to j$}
		\STATE $h_{ij} = (\vec{v}_{j},\vec{w}_{i})$
		\STATE $\vec{v}_{j} = \vec{v}_{j} - h_{ij}\vec{w}_{i}$
	\ENDFOR
	\STATE $h_{j+1,j} = \|\vec{v}_{j}\|$ If $h_{j+1,j} = 0$ set $m=j$ and go to $10$
	\STATE $\vec{w}_{j+1}=\vec{v}_{j}/h_{j+1,j}$
\ENDFOR
\STATE Define the $(m+1)\times m$ Hessenberg matrix $\bar{\mathbf{H}}_{m}$
\STATE Compute $\vec{y}_{m}$ the minimizer of $\|\beta\vec{e}_{1} - \bar{\mathbf{H}}_{m}\vec{y}\|$
\STATE Compute approximate solution $\vec{x}_{m} = \vec{x}_{0}+\mathbf{W}_{m}\vec{y}_{m}$
\end{algorithmic}
\label{algo:gmres}
\end{algorithm}
% subsection gmres_an_example_of_a_krylov_method (end)
% section krylov_methods (end)

\section{Approximate eigenvectors of $\mathbf{M}_{BD}\,\mathbf{A}$}\label{app:aprox_eigenvector}

In this Appendix we outline the Ritz approach to approximating
eigenvectors of a matrix. More details of this technique in the
context of preconditioning linear systems of equations can be found
in~\citet{ADDM}.

We begin with solving the linear system, $\mathbf{A}\,\vec{x}  = 
\vec{b}$, as given in Equations~\eqref{eq:Sdef}-\eqref{eq:rhs}, by using a Krylov
subspace solver.  Following~\citet{ADDM}, we assume that this is done
with the GMRES algorithm, though similar
considerations apply as well to CG~\citep[see for instance][]{ACG}.
We denote the number of iterations needed to converge to the solution
as $m$ and assume that the standard preconditioner
$\mathbf{M}_{BD}$ is applied in the course of the procedure.

The relevant Krylov space for the system with the preconditioned
matrix $\mathbf{B} := \mathbf{M}_{BD}\mathbf{A}$ and corresponding, initial residual $\vec{r}_{0}:= \mathbf{M}_{BD}(\vec{b} - \mathbf{A}\vec{x}_{0})$ is defined as,
\begin{eqnarray}\label{eq:krylov_block_prec}
	\mathcal{K}_{m}( \mathbf{B} , \vec{r}_{0})=\text{SPAN}\left\{\vec{r}_{0},\mathbf{B} \vec{r}_{0}, \mathbf{B}^{2}\vec{r}_{0},\ldots, \mathbf{B}^{m-1}\vec{r}_{0} \right\}
\end{eqnarray}
As described in details in previous section, the GMRES algorithm uses the
Arnoldi iterations (see algorithm~\ref{algo:arnoldi}) to compute the
orthonormal basis $\mathbf{W}$ of the Krylov space together
with a set of scalar coefficients $h_{ij}$ (where $ i,j = 1, \dots,
m$ and $i \le j+1$), plus an extra coefficient, $h_{m+1,m}$. The first
group of the coefficients can be arranged as a square matrix of rank
$m$, a sub-operator created from of the Hessenberg matrix which we will denote $\mathbf{H}$. We can relate this operator with a fundamental
relation between products of the Arnoldi process and Hessenberg matrix define in equation~\eqref{eq:arnoldi_fundamental}, which now
reads,
\begin{eqnarray}\label{eq:arnoldi}
\mathbf{B}\,\mathbf{W}_{m}\,=\, \mathbf{W}_{m+1}\bar{\mathbf{H}}_{m}\,=\,\mathbf{W}_{m}\,\mathbf{H}_{m}\,+\,h_{m+1,m}\,\vec{w}_{m+1}\vec{e}^{\dagger}_{m}.
\end{eqnarray}
Here, $\vec{e}_m$ is a unit vector with $1$ on the $m$th place.
The eigenpairs of the matrix $\mathbf{H}_m$ are commonly referred to
as Ritz eigenpairs.  They can be straightforwardly computed thanks to
its upper-triangular structure and moderate size, which is given by
the size of the Krylov space and therefore by the typical number of the
iterations needed to solve the system. This in in the CMB applications is on the order of ${\cal
  O}(100)$.  By denoting these eigenpairs as $(\vec{g}_i,\lambda_i)$,
we can therefore write,
\begin{eqnarray}
\mathbf{H}_m\,\vec{g}_i \, = \, \lambda_i \, \vec{g}_i.
\end{eqnarray}
From Eq.~\eqref{eq:arnoldi}  for every eigenvector, $\vec{g}_i$, of $\mathbf{H}_m$, we find that,
\begin{eqnarray}
\mathbf{B}\,\mathbf{W}_m\,\vec{g}_i \, & = &  \, \mathbf{W}_m\,\mathbf{H}_m\,\vec{g}_i \, + \, h_{m+1, m}\,\vec{w}_{m+1}\,\vec{e}^\dagger_m\,\vec{g}_i\nonumber \\
& = & \, \lambda_i \, \mathbf{W}_m\, \vec{g}_i \, + \, h_{m+1, m}\,\vec{w}_{m+1}\,\vec{e}^\dagger_m\,\vec{g}_i.
\label{eq:approxEigen}
\end{eqnarray}
Consequently, if $h_{m+1, m} = 0$ then every eigenvector of $\mathbf{H}_m$ defines an eigenvector of $\mathbf{B}$ given by $\vec{y}_i := \mathbf{W}_m\,\vec{g}_i$,  both of which have the same corresponding eigenvalue, $\lambda_i$. 

If $h_{m+1, m}$ is not zero, but is small, as it is usually the case if the solver converged with sufficient precision, then the pairs $(\vec{y}_i, \lambda_i)$ provide a useful approximation of the $m$ true eigenvalues of $\mathbf{B}$, and the magnitude of the last term on the right hand side of Eq.~\eqref{eq:approxEigen} serves as an estimate of the involved error. 

Consequently, in our construction of the {\em a posteriori} preconditioner we use suitable defined subsets of vectors $\vec{y}_i$ to build the deflation subspace operator, $\mathbf{Z}_D$.

%\section{Deflation}\label{sec:app_deflation} % (fold)
%In this section we briefly describe a main idea behind deflation, a know approach for convergence acceleration of Krylov methods. In \emph{deflation} the system $\mathbf{A} \vec{x} = \vec{b}$ is multiply with a suitably chosen projection, and the general goal is to "eliminate" components that supposedly slow down convergence. Typically there are components that corresponds to small eigenvalues. In this context deflation is used to improve condition number by shifting some of the smallest eigenvalues to zero. Since the corresponding eigenvectors no longer have components during the iterations, Krylov method will converge faster. Here, we can speak of the \emph{effective} condition number after deflation, is is never larger than the \emph{original} condition number. 
%
%To demonstrate deflation preconditioners, we define following operators:
%\begin{eqnarray}\label{eq:projection_definition}
%\mathbf{R} := \mathbf{I} - \mathbf{A}\,\mathbf{Z}\, \mathbf{E}^{-1}\,\mathbf{Z}^{T},\,\mathbf{Q} := \mathbf{I} - \mathbf{Z}\, \mathbf{E}^{-1}\,\mathbf{Z}^{T}\,\mathbf{A},\,\mathbf{E} := \mathbf{Z}^{T}\mathbf{A}\,\mathbf{Z},
%\end{eqnarray}
%where $\mathbf{R}$ and $\mathbf{Q}$ are related to the left and right preconditioner, respectively. One can easily show that $\mathbf{R}$ and $\mathbf{Q}$ are projectors, i.e., $\mathbf{R}^{2}=\mathbf{R}$ and $\mathbf{Q}^{2}=\mathbf{Q}$. Here, $\mathbf{Z}$ is a suitable deflation subspace of dimension $n \times r$, which $r \ll n$, end hence $\mathbf{E}$ is presumable easy to compute and invert. With those operators, the solution $\vec{x}$ of our original linear system $\mathbf{A} \vec{x} = \vec{b}$ can be now rewritten:
%\begin{equation}
%	\vec{x} = (\mathbf{I} - \mathbf{Q})\vec{x} + \mathbf{Q}\vec{x} = \mathbf{Z}\mathbf{E}^{-1}\mathbf{Z}^{T}\vec{b} + \mathbf{Q}\vec{x}.
%\end{equation}
%As the first term in the right-hand side is easy to compute, the factor $\mathbf{Q}\vec{x}$ is then obtained by computing $\widetilde{\vec{x}}$ from
%\begin{equation}\label{eq:deflation_sys}
%	\mathbf{R}\widetilde{\vec{x}} = \mathbf{R}\vec{b}
%\end{equation}
%and then premultiplying is with $\mathbf{Q}$. Although the deflated matrix $\mathbf{R}\mathbf{A}$ is singular, the deflated linear system~\eqref{eq:deflation_sys} is consistent  because the same projection is apply to both sides. Hence, it can be solved by an appropriate Krylov subspace method. In this case, the search space of the Krylov subspace method applied to~\eqref{eq:deflation_sys} can be rewritten as
%\begin{equation}
%	\widetilde{\mathcal{K}}_{m} = \mathcal{K}_{m}( \mathbf{R}\,\mathbf{A} , \mathbf{R}\,\vec{r}_{0})
%\end{equation}
%while the current approximate solution $\widetilde{\vec{x}}_{m}$ and the current residual $\widetilde{\vec{r}}_{m} = \mathbf{R}(\vec{b} - \mathbf{A}\,\widetilde{\vec{x}}_{m})$ at the end of iterative process satisfies the relations
%\begin{eqnarray}
%	\widetilde{\vec{x}}_{m}  & \in &	\widetilde{\vec{x}}_{0} + \widetilde{\mathcal{K}}_{m} \\
%	\mathbf{R}(\vec{b} - \mathbf{A}\,\widetilde{\vec{x}}_{m}) & \bot & \mathbf{R}\,\mathbf{A}\,\mathcal{K}_{m}( \mathbf{R}\,\mathbf{A} , \mathbf{R}\,\vec{r}_{0}).
%\end{eqnarray}
%
%Since $\mathbf{R}\,\mathbf{A}\,\mathbf{Z} = 0_{n\times r}$, $\mathbf{R}\,\mathbf{A}$ is singular. Therefore, it is of greatest importance to analyze the possibilities of a breakdown due to round-off errors when solving the deflated linear system~\eqref{eq:deflation_sys}. This feature has been notably analyzed in~\citep{Gutknecht_spectraldeflation}, based on theoretical results obtained by~\cite{Brown_Walker}.
% subsection definition (end)
% section deflation (end)


==> sections_post_sub/sec_prec_algebra.tex <==
%!TEX root = ../midas_preconditioner.tex 

\section{Speed of iterative inversion}\label{sec:two-level-prec}

It is well known~\citep[see][]{CGfirst,sluis86} that the convergence rate of the conjugate gradient method is bounded in terms of the condition number of $A$, i.e., after $j$ iterations of CG, we have
\begin{equation}\label{eq:err_bound}
	\|{\vec{x}}-{\vec{x}}_{j}\| \leq 2 \| {\vec{x}} - {\vec{x}}_{0} \|_{A}\left(\frac{\sqrt{\kappa}-1}{\sqrt{\kappa}+1}\right)^{j},
\end{equation}
where ${\vec{x}}_{0}$ is the starting vector and $\|\vec{x}\|_{A}$ is a $A$-norm of $\vec{x}$, defined as $\|\vec{x}\|_{A}=\sqrt{\vec{x}^{T}A\vec{x}}$. The effective condition number $\kappa = \kappa(A)$ is defined as ratio of the largest to smallest positive eigenvalue $\lambda_{i}$ of matrix $A$. If $\kappa$ is large, it is more favourable to solve preconditioned system $M\,A{\vec{x}} = M\,\vec{b}$ instead of~\eqref{eq:linear_system}, where symmetric positive definite preconditioner $M$ is chosen such that $M\,A$ has more clustered spectrum or a smaller condition number then that of $A$. 

To date, the issue of efficient preconditioner for map making problem has been left largely intact with nearly all performed
studies relying on the PCG solver
and invoking the same, intuitive, easy to compute and implement
preconditioner~\citep{madmap}, given as,
\begin{eqnarray}\label{eq:stdPrec}
M := M_{BD} = \left[ \mathbf{P}^{T} \, {\rm diag}\, (N^{-1}) \, \mathbf{P}\right]^{-1}.
\end{eqnarray}
Here ${\rm diag}\, (N^{-1}) $ is a diagonal matrix consisting of the 
diagonal elements of $N^{-1}$. $M_{BD}$ coincides with the inverse of the coefficient matrix of our
system, $A$, whenever the time domain noise is white and therefore can
be expected to provide a satisfactory approximation to $A^{-1}$ also in more
general cases and therefore be efficient as a preconditioner.  We note that given the assumptions
made here about the matrix $\mathbf{P}$,  $M_{BD}$ is block diagonal with dimension of block equal to number of Stokes parameters (usually 3). Therefore we will
refer to it in the following either as the standard or block diagonal preconditioner. 

To motivate the choice new preconditioner for this
research, let us first have a brief look at strengths and weakness of
the standard preconditioner $M_{BD}$.  Some insight into this
can be obtained by analyzing the spectrum of the preconditioned system
coefficient matrix, i.e., $M_{BD}\, A$, and compare it with the spectrum
of the matrix $A$ alone. An example of such a comparison computed for
one of the experiments studied in~\S\ref{sec:numerical_experiments} is shown in figure
\ref{fig:eigen_values}.  As it is clear from the figure, the
preconditioner performs very well as far as the very large eigenvalues
of the initial matrix are concerned, suppressing them uniformly to
nearly a unity. At the same time, however, its small eigenvalues
become even smaller and thus continue to hinder the convergence of the
iterative method.

This problem can be solved by a deflation technique e.g.,~\citep{Nicolaides:1987,TANG:2009} which bases on the usage of a projection operator 
\begin{equation}\label{eq:projection}
	R = I - A Z\left(Z^{T}A Z\right)^{-1}Z^{T}\,,
\end{equation}
in construction of more efficient preconditioner. The column space $Z\in\mathbb{R}^{{\cal N}_p\times r}$ is the so-called the deflation subspace, i.e., the space to be projected out of the residual, and $I$ is the identity matrix of appropriate size. We assume that $r \ll {\cal N}_{p}$ and that $Z$ has rank $r$. Under this assumption the coarse operator $E := Z^{T}AZ$ may be easily computed and factored and moreover, $E$ is symmetric positive definite. Since ${\vec{x}} = (I-R^{T}){\vec{x}} + R^{T}{\vec{x}}$. 

In order to improve conditioning of the coefficient matrix, the projection operator $R$ is usually combine with traditional preconditioner, so that the resulting approach gets rid of the effect of both small and large eigenvalues. For instance, it can be proved~\citep[see][Theorem 2.2]{Vui06NT} that
\begin{equation}
	\kappa(M_{BD}RA) < \kappa(M_{BD}A),
\end{equation}
for any $M_{BD}$ being a SPD matrix. This combined preconditioning is know as 'two-level preconditioning', and many different version can be found in literature. Our two-level preconditioner is based on the
adapted deflation preconditioner introduced in~\citep{TANG:2009},
\begin{eqnarray} \label{eq:2}
{\mathcal M}_{2lvl} & := & M_{BD}\,R  + ZE^{-1}Z^{T} = M_{BD}\left(I - AZE^{-1}Z^{T}\right) + ZE^{-1}Z^{T}\,,
\end{eqnarray}
and combines the effect of the block diagonal preconditioner~\eqref{eq:stdPrec} on the higher part of the spectrum with a coarse space correction of the lower part
of the spectrum.

Compared to the diagonal preconditioner $M_{BD}$, the two-level
preconditioner introduces unavoidably an additional numerical cost,
which is however manageable as it corresponds mainly to solving a small
linear system with the matrix $E$ (see
section~\ref{sec:parall-constr-coarse} for a more detailed
discussion).





